DeepMLF: Multimodal language model with learnable tokens for deep fusion in sentiment analysis

While multimodal fusion has been extensively studied in Multimodal Sentiment Analysis (MSA), the role of fusion depth and multimodal capacity allocation remains underexplored. In this work, we position fusion depth, scalability, and dedicated multimodal capacity as primary factors for effective fusion. We introduce DeepMLF, a novel multimodal language model (LM) with learnable tokens tailored toward deep fusion. DeepMLF leverages an audiovisual encoder and a pretrained decoder LM augmented with multimodal information across its layers. We append learnable tokens to the LM that: 1) capture modality interactions in a controlled fashion and 2) preserve independent information flow for each modality. These fusion tokens gather linguistic information via causal self-attention in LM Blocks and integrate with audiovisual information through cross-attention MM Blocks. Serving as dedicated multimodal capacity, this design enables progressive fusion across multiple layers, providing depth in the fusion process. Our training recipe combines modality-specific losses and language modelling loss, with the decoder LM tasked to predict ground truth polarity. Across three MSA benchmarks with varying dataset characteristics, DeepMLF achieves state-of-the-art performance. Our results confirm that deeper fusion leads to better performance, with optimal fusion depths (5-7) exceeding those of existing approaches. Additionally, our analysis on the number of fusion tokens reveals that small token sets ($\sim$20) achieve optimal performance. We examine the importance of representation learning order (fusion curriculum) through audiovisual encoder initialization experiments. Our ablation studies demonstrate the superiority of the proposed fusion design and gating while providing a holistic examination of DeepMLF's scalability to LLMs, and the impact of each training objective and embedding regularization.

==> tex/method_old.tex <==
\section{\textit{msa}GPT}
\label{sec:method}




Our proposed multimodal regularization method, \ours, is described here in detail. It consists of five key elements:
\begin{enumerate}
	\item Generating a \emph{varying number of mixed examples}.
	\item \emph{Mixing factor reweighting}, adjusting the contribution of each representation in a mixed example.
	\item \emph{Anisotropic mixing}, \ie, sampling distinct mixing factors for each latent modality space.
	\item \emph{Dynamic mixing}, allowing the combination of a variable number of embeddings from the mini-batch.
	\item \emph{Cross-modal label mixing}, creating a unified multimodal label for each mixed multimodal tuple.
\end{enumerate}
While the first two elements build upon established concepts in the literature (see \autoref{sec:multimix} and \autoref{sec:repr_reweight} respectively), the other three are entirely novel contributions, specifically designed to make \ours perform best in a multimodal setup. In the following, we provide a detailed account of how \ours combines these novel elements in a multi-step algorithm, and then we discuss their motivation and impact. We give pseudo-code for \ours in \autoref{alg:powmix}.

% 1) Importance-based reweighting, which adjusts the significance of each representation;
% 2) A dynamic mixing process, enabling the combination of a variable number of embeddings for increased flexibility;
% 3) Generation of a varying number of mixtures;
% 4) Anisotropic mixing, i.e., sampling distinct mixing factors for each modality;
% and
% 5) cross-modal label mixing, creating a unified multi-modal label for each mixed multimodal tuple.

%------------------------------------------------------------------------------
\begin{algorithm}
\small

\SetFuncSty{textsc}
\SetDataSty{emph}
\newcommand{\commentsty}[1]{{\color{ForestGreen}#1}}
\SetCommentSty{commentsty}
\SetKwComment{Comment}{$\triangleright$ }{}

\KwIn{hidden representations $\vH_m \in \real^{B \times d_m}$}
\KwIn{label vector $\vy \in \real^B$}
\KwIn{number $n_O$ of generated mixed examples}
\KwOut{mixed representations $\wt{\vH}_m \in \real^{n_O \times d_m}$}
\KwOut{mixed label vector $\wt{\vy} \in \real^{n_O}$}

$\va_m \gets g_A(\vH_m)$ \Comment*[f]{attention vector} \\
$\valpha_m \sim U(0.5, 2)$ \Comment*[f]{interpolation hyperparameter} \\
$\vLambda_{m} \sim \Dir(\valpha_m)$ \Comment*[f]{interpolation matrix} \\
$\vP \sim U(2, 4)$ \Comment*[f]{masking hyperparameter} \\
$\vM \sim \Bern(\vP / B)$ \Comment*[f]{mask sampling} \\
$\wt{\vLambda}_m \gets \eta_1(\va_m\tran \odot \vM \odot \vLambda_m)$ \Comment*[f]{normalization} \\
$\wt{\vH}_m \gets \wt{\vLambda}_m \vH_m$ \Comment*[f]{representation mixing} \\
$\wt{\vy}_m \gets \wt{\vLambda}_m \vy_m$ \Comment*[f]{label mixing} \\
$\wt{\vy} \gets \frac{1}{M} \sum_m \wt{\vy}_m$ \Comment*[f]{cross modal label mixing}

\caption{\ours multimodal mixing.}
\label{alg:powmix}
\end{algorithm}
%------------------------------------------------------------------------------

\subsection{Algorithm}
\label{sec:powmix_overview}

Given a multimodal example $\vX^{(i)} = (\vX^{(i)}_1, \dots, \vX^{(i)}_M) \in \cX_\cM$, we obtain a hidden representation $\vh^{(i)}_m = f_m(\vX^{(i)}) \in \real^{d_m}$ as the output of encoder $f_m$ for each modality $m \in \cM$. At the mini-batch level, let the matrix $\vH_m \in \real^{B \times d_m}$ hold the hidden representations of all examples in its rows, where $B$ is the mini-batch size. Let also vector $\vy \in \real^B$ denote the labels $y^{(i)} \in \real$ for all examples of the mini-batch.

\paragraph*{Mixing factor reweighting}

First we compute the \emph{mixing factor attention weights} $\va_m \in \real^B$. Specifically, as a form of attention, we use average pooling over the feature dimension followed by ReLU and normalization across modalities:
\begin{equation}
	\va_m = g(\vH_m) \defn
		\frac{\sigma(\vH_m \vone_{d_m} / d_m)}{\sum_{m'} \sigma(\vH_{m'} \vone_{d_{m'}} / d_{m'})},
\label{eq:attention}
\end{equation}
where $\vone_{d_m} \in \real^{d_m}$ is an all-ones vector, $\sigma(\cdot)$ is the ReLU function and  division is performed element-wise. This operation is similar to transformer cross-attention between query $\vone_{d_m}$ and key $\vH_m$ but here normalization is performed across modalities. We call the use of weights $\va_m$ \emph{mixing factor reweighting}. A baseline is to use a uniform $\va = \vone_B / M$ for all modalities.

\paragraph*{Anisotropic mixing}

For each modality, we then sample a different \emph{mixing matrix} $\vLambda_m \in \real^{n_O\times B}$. To do this, we sample $n_O$ distinct $B$-dimensional interpolation coefficient vectors from a Dirichlet distribution $\Dir(\valpha_m)$, with its parameter $\valpha_m \in \real^{n_O}$ drawn from a uniform distribution $U(0.5, 2.0)$, following~\cite{venkataramanan2023Embedding}. Let's assume that the latentrepresentation of each modality is embedded in separate subspaces of an overall multimodal latent representation space. Since we use a different mixing matrix per subspace, we call this approach \emph{anisotropic mixing}. A simpler alternative is to use the same $\vLambda \in \real^{n_O\times B}$ for all modalities.

\paragraph*{Dynamic mixing}

Next, we randomly mask mixing factors to keep only a small number of nonzero elements per row of $\vLambda_m$. This limits the interpolation to just a few examples. Specifically, we sample a binary mask $\vM \sim \Bern(\vP / B) \in \real^{n_O\times B}$ from a Bernoulli distribution and apply it element-wise to the mixing matrix $\vLambda_m$.

The hyperparameter $\vP \in \real^{n_O \times B}$ provides a different value for each element of $\vM$ and dictates the proportion of mini-batch examples to interpolate in the representation space. We find empirically that $\vP \sim U(2, 4)$ works well, corresponding to $2$ to $4$ nonzero elements on average per row of $\vLambda_m$.

Since different examples are interpolated for each generated example, we call this process \emph{dynamic mixing}. Importantly, the same binary mask $\vM$ is used for all modalities $m$ by default, a choice called \emph{mask sharing}. An alternative is to use a different $\vM_m \in \real^{n_O\times B}$ for each modality. The simplest approach would be not to use any masking, \ie setting $\vM = \vone_{n_O \times B}$, which deactivates dynamic mixing. 

\paragraph*{Interpolation operation}

Given the mixing factor attention weights $\va_m \in \real^B$ and the binary mask $\vM \in \real^{n_O\times B}$, we multiply element-wise with the mixing matrix $\vLambda_m \in \real^{n_O\times B}$ and re-normalize over the mini-batch dimension to obtain the \emph{reweighted mixing matrix}
\begin{equation}
	\wt{\vLambda}_m = \eta_1(\va_m\tran \odot \vM \odot \vLambda_m) \in \real^{n_O\times B},
\label{eq:mixing_factor_reweighting_powmix}
\end{equation}
where $\eta_1$ here denotes $\ell_1$-normalization of rows and $\odot$ is Hadamard product (with vectors broadcasting to matrices as needed). In this product, attention weights $\va_m$ are scaling the columns of the mixing matrix, while the binary mask $\vM$ is selecting subsets from each row.

Now, using $\wt{\vLambda}_m$, we generate $n_O$ mixed examples per modality. In particular, given the hidden representations $\vH_m$ and the labels $\vy$, we perform intra-modal interpolation for modality $m$ by
\begin{align}
	\wt{\vH}_m &= \wt{\vLambda}_m \vH_m \in \real^{n_O \times d_m} \label{eq:powmix_h} \\
	\wt{\vy}_m &= \wt{\vLambda}_m \vy \in \real^{n_O}. \label{eq:powmix_y}
\end{align}
This is similar with~\eq{multimix_h}, \eq{multimix_y}, but $\wt{\vLambda}_m$ is reweighted, masked and unique for each modality. Formally, it expresses convex combinations of different input examples in the representation space and their labels, due to nonnegativity of $\wt{\vLambda}_m$ and its rows summing to $1$.

\paragraph*{Cross-modal label mixing}

Finally, we compute a single multimodal label $\wt{\vy} \in \real^{n_O}$ for the mini-batch by averaging $\wt{\vy}_m$ over modalities:
\begin{equation}
	\wt{\vy} = \frac{1}{M} \sum_m \wt{\vy}_m.
\label{eq:cross-modal_label_mixing}
\end{equation}
This step, called \emph{cross-modal label mixing}, is only meaningful when mixing factor reweighting and anisotropic mixing are used, in which case $\wt{\vy}_m$ are different for each modality.

%------------------------------------------------------------------------------

\subsection{Discussion}
\label{sec:method-discussion}

We now discuss the key features of \ours, to better understand the underlying idea of each algorithmic component.

\paragraph*{Varying number of mixed examples}

\ours enables the generation of a variable number $n_O$ of mixed examples. These mixtures lie in the convex hull of the mini-batch in the representation space. 
The value of $n_O$ is a hyperparameter, which is decoupled from the mini-batch size and much larger in practice. 
As such, it generates a plethora of mixtures, leading to more loss terms being calculated per example during model training.
As in MultiMix~\cite{venkataramanan2023Embedding}, it is hypothesized that this provides a better approximation of the expected risk integral.

\paragraph*{Mixing factor reweighting}

Prior works~\cite{transmix, venkataramanan2023Embedding} perform mixing factor reweighting on dense features of image patches, applied to a unimodal task. By contrast, our approach is inherently multimodal, reweighting the mixing factors of each mini-batch example by normalizing across modalities. 
Our intuition is that by reweighting each modality in a multimodal $m$-tuple according to the sum of its features we are able to reduce the impact of uninformative (near zero) unimodal instances in the representation space.  
Unlike prior work~\cite{transmix, venkataramanan2023Embedding}, our approach is also agnostic to the architecture and pooling mechanism of the input modality encoders. We experimentally verify that it improves performance.

\paragraph*{Anisotropic mixing}

Given $m$ hidden tensors $\vH_m \in \real^{B\times d_m}$, \ours samples a separate mixing matrix $\vLambda_m \in \real^{n_O \times B}$ for each modality $m$. This enables modality-specific mixing, that is, the ability of the algorithm to exhibit different mixing strategies across modalities. This property is shown to be critical for \ours to perform well.

\paragraph*{Dynamic mixing and power set}

Considering the formation of the reweighted mixing matrix $\wt{\vLambda}_m$~\eq{mixing_factor_reweighting_powmix}, we track two sources of randomness. The first is due to mixing factors in $\vLambda_m$, sampled from the Dirichlet distribution, which is common in prior mixing methods, \eg~\cite{venkataramanan2023Embedding}.
The second is due to the binary mask $\vM$, sampled from the Bernoulli distribution, which is unique to our method. 
One may interpret the interpolation process as sampling a subset of examples from the \emph{power set} $\cP$ of the mini-batch in the representation space. The subset sampling is then followed by the formation of a convex combination based on the selected representations. 
This is a \emph{dynamic mixing} process in the sense of using a different subset for each generated mixed example. 
The \ours acronym of  the proposed method  alludes to the use of the power set $\cP$.

In practice, the effect of sampling a subset prior to forming a convex combination is that $\wt{\vLambda}_m$ is \emph{sparse}, having a small number of nonzero entries per row (2 to 4 on average according to our default settings). Thus, only few mini-batch examples are interpolated for each generated mixture. 
While it is possible to control the entropy of mixing factors by adjusting the hyperparameter $\valpha_m$ of the Dirichlet distribution in sampling $\vLambda_m$ itself, it is shown experimentally that true sparsity is superior in our multimodal problem. 
As shown in \autoref{fig:powmix_3} and \autoref{fig:powmix_4}, \ours can provide mixing instances between interpolation of \emph{pairs}, as in Manifold Mixup~\cite{verma2019manifold}, and \emph{all} mini-batch examples, as in MultiMix~\cite{venkataramanan2023Embedding}. 
Sharing the binary mask $\vM$ across modalities is empirically shown to be essential for \ours to work well.

\paragraph*{Cross-modal label mixing}

\ours uses mixing factor reweighting and anisotropic mixing, which result in different reweighted mixing matrices $\wt{\vLambda}_m$~\eq{mixing_factor_reweighting_powmix} and thus different mixed labels $\wt{\vy}_m$~\eq{powmix_y} for each modality $m$.
To unify these into a single label vector $\wt{\vy}$, \ours averages the mixed labels $\wt{y}_m$ over modalities~\eq{cross-modal_label_mixing}. This assumes equal contribution from each modality in label generation.
While this assumption may not hold universally, empirical evidence has demonstrated its effectiveness in practice.
% \iavr{Could have tried to use attention per example per modality like~\eq{attention} \emph{after} mixing?}
The averaging operation is purely multimodal, intertwining label information across different modalities.


